ISimDL: Importance Sampling-Driven Acceleration of Fault Injection Simulations for Evaluating the Robustness of Deep Learning

Deep Learning (DL) systems have proliferated in many applications, requiring specialized hardware accelerators and chips. In the nano-era, devices have become increasingly more susceptible to permanent and transient faults. Therefore, we need an efficient methodology for analyzing the resilience of advanced DL systems against such faults, and understand how the faults in neural accelerator chips manifest as errors at the DL application level, where faults can lead to undetectable and unrecoverable errors. Using fault injection, we can perform resilience investigations of the DL system by modifying neuron weights and outputs at the software-level, as if the hardware had been affected by a transient fault. Existing fault models reduce the search space, allowing faster analysis, but requiring a-priori knowledge on the model, and not allowing further analysis of the filtered-out search space. Therefore, we propose ISimDL, a novel methodology that employs neuron sensitivity to generate importance sampling-based fault-scenarios. Without any a-priori knowledge of the model-under-test, ISimDL provides an equivalent reduction of the search space as existing works, while allowing long simulations to cover all the possible faults, improving on existing model requirements. Our experiments show that the importance sampling provides up to 15x higher precision in selecting critical faults than the random uniform sampling, reaching such precision in less than 100 faults. Additionally, we showcase another practical use-case for importance sampling for reliable DNN design, namely Fault Aware Training (FAT). By using ISimDL to select the faults leading to errors, we can insert the faults during the DNN training process to harden the DNN against such faults. Using importance sampling in FAT reduces the overhead required for finding faults that lead to a predetermined drop in accuracy by more than 12x.

==> config/paper/ieeetran_conference/predoc_config.tex <==
% The following line is only needed to identify funding in the first footnote.
% If that is unneeded, please comment it out.
% it is required for \thanks in the author
% must be enabled before \begin{document}
% \IEEEoverridecommandlockouts

% to modify the spacing before the title, modify this value
% this is overwritten by ieeeconf_ras_compatibility if it is required
\renewcommand{\IEEEtitletopspaceextra}{0pt}


==> config/paper/ieeetran_ras/predoc_config.tex <==
% The following line is only needed to identify funding in the first footnote.
% If that is unneeded, please comment it out.
% it is required for \thanks in the author
% must be enabled before \begin{document}
% \IEEEoverridecommandlockouts

% needed to meet printer requirements
% IROS template, only for use with ieeeconf
% \overrideIEEEmargins

\import{config/paper/ieeetran_ras/compatibility/}{ieeetran_compatibility_ieeeconf_ras_config_predoc}


==> content/paper/sections/0_round0.tex <==
\section{Round 0}


\textbf{Idea:} Importance Sampling acceleration of fault injection, with fault-aware training as use case


\textbf{Novel contributions:}
\begin{itemize}
    \item importance sampling based on output/weight importance
    \item ??? fault-aware training use case for importance sampling
    \item comparison of importance and random sampling regarding convergence speed, diversification
    \item comparison of full importance sampling (bit position and neuron position are based on weights) to partial importance sampling (only bit position is based on weights) to full random sampling
\end{itemize}

% why SotA has not addressed this yet, what are the challenges
\textbf{Scientific Challenges:}
\begin{itemize}
    \item missing proper fault injection framework optimized for fast execution (enpheeph, LLFI)
    \item 
    \item 
\end{itemize}

\textbf{Current Results:}
\begin{itemize}
    \item Better than state-of-the-art
    \begin{itemize}
        \item Wider coverage in same amount of time
        \item Faster convergence for same number of critical faults
    \end{itemize}
    \item Similar accuracy/fault coverage as state-of-the-art
\end{itemize}

\textbf{Comparison with SotA:}
\begin{itemize}
    \item Comparison with random sampling, both for convergence speed and coverage of faults for bad errors
\end{itemize}

\textbf{Expected Results:}
\begin{itemize}
    \item fault-aware training? Comparison with normal random sampling for fault collection on the newly trained network, faster convergence wins
    \item 
\end{itemize}

==> content/paper/sections/a_acknowledgment.tex <==
\section*{Acknowledgment}
\label{section:acknowledgment}

==> content/paper/to_appear_header.tex <==
\setuptoappearheader{To appear at the 24th IEEE/ACM Design, Automation and Test in Europe (DATE'21) Conference, February, 2021}
\toappearheader
